AnyECG: Foundational Models for Multitask Cardiac Analysis in Real-World Settings

Electrocardiogram (ECG), a non-invasive and affordable tool for cardiac monitoring, is highly sensitive in detecting acute heart attacks. However, due to the lengthy nature of ECG recordings, numerous machine learning methods have been developed for automated heart disease detection to reduce human workload. Despite these efforts, performance remains suboptimal. A key obstacle is the inherent complexity of ECG data, which includes heterogeneity (e.g., varying sampling rates), high levels of noise, demographic-related pattern shifts, and intricate rhythm-event associations. To overcome these challenges, this paper introduces AnyECG, a foundational model designed to extract robust representations from any real-world ECG data. Specifically, a tailored ECG Tokenizer encodes each fixed-duration ECG fragment into a token and, guided by proxy tasks, converts noisy, continuous ECG features into discrete, compact, and clinically meaningful local rhythm codes. These codes encapsulate basic morphological, frequency, and demographic information (e.g., sex), effectively mitigating signal noise. We further pre-train the AnyECG to learn rhythmic pattern associations across ECG tokens, enabling the capture of cardiac event semantics. By being jointly pre-trained on diverse ECG data sources, AnyECG is capable of generalizing across a wide range of downstream tasks where ECG signals are recorded from various devices and scenarios. The experimental results show that AnyECG achieves an average performance improvement of 6% across four critical tasks-anomaly detection, arrhythmia classification, corrupted lead generation, and ultra-long ECG recognition. AnyECG learns common ECG rhythm from data and significantly outperforms state-of-the-art methods in each of these tasks.

==> sec/1.abstract.tex <==
\begin{abstract}
% The electrocardiogram (ECG) is a widely used biosignal for cardiac monitoring, but its analysis faces significant challenges due to varied acquisition methods, inconsistent signal lengths, and mismatched channels across datasets. Additionally, the low signal-to-noise ratio characteristic of ECG signals also makes it more difficult for deep learning models to obtain representations of ECG signals. To overcome these challenges, we propose a foundational model for ECG signal representation, named ECGFM. \model  employs a flexible ECG tokenizer architecture that segments ECG signals into patches and uses vector-quantized ECG rhythm prediction to train the Patient Attribute Tokenizer. This tokenizer encodes raw ECG patches into compact rhythm codes, capturing spatial and temporal features of the ECG signals. Then, we pre-train \model using a masked-attention architecture by predicting missing tokens and patient attribute information, enabling cross-dataset learning. 

% This self-supervised learning approach encourages the model to learn general representations of ECG signals, enhancing its applicability across diverse datasets and tasks.  We evaluated ECGFM on downstream tasks such as arrhythmia classification and diagnostics, where it consistently outperformed baseline models, demonstrating superior generalization.  Our experiments validate the effectiveness of ECGFM in handling heterogeneous ECG data.  The code is available at XXX.



% Electrocardiography (ECG) is a non-invasive and cost-effective tool widely used for cardiac monitoring and the diagnosis of heart diseases. Its ability to provide real-time insights into the heart's electrical activity makes it invaluable in both clinical and home settings. However, analyzing ECG data presents significant challenges due to heterogeneity in acquisition methods—differences in equipment, signal properties, lead configurations, sampling frequencies, and patient demographics across various datasets. Additionally, the low signal-to-noise ratio characteristic of ECG signals also makes it more difficult to obtain representations of ECG signals. 
% % These challenges collectively limit the full potential of large-scale ECG data analysis.

% To overcome these challenges, we propose ECGFM, a foundational model developed for ECG signal representation that generalizes across diverse datasets.  \model divides ECG signals into patches of uniform length, enabling learning across heterogeneous data. Then \tokenizer transforms continuous and noisy ECG patches into compact and meaningful tokens, effectively addressing the low signal-to-noise ratio issue. Finally, to learn the real meanings and interrelationships of these tokens, as well as their relationships across different datasets, we train the model by predicting the tokens of masked ECG patches.  This approach enhances its applicability across different datasets and tasks, enabling ECGFM to effectively handle heterogeneous ECG data. In downstream tasks such as arrhythmia classification and diagnostics, ECGFM consistently outperforms baseline models, demonstrating superior generalization and performance. Our experimental results validate the effectiveness of ECGFM in dealing with diverse ECG datasets. The code is available at XXX.
Electrocardiogram (ECG), a non-invasive and affordable tool for cardiac monitoring, is highly sensitive in detecting acute heart attacks. However, due to the lengthy nature of ECG recordings, numerous machine learning methods have been developed for automated heart disease detection to reduce human workload. Despite these efforts, performance remains suboptimal. A key obstacle is the inherent complexity of ECG data, which includes heterogeneity (\textit{e.g.}, varying sampling rates), high levels of noise, demographic-related pattern shifts, and intricate rhythm-event associations.
To overcome these challenges, this paper introduces {\model}, a foundational model designed to extract robust representations from any real-world ECG data. Specifically, a tailored {\tokenizer} encodes each fixed-duration ECG fragment into a token and, guided by proxy tasks, converts noisy, continuous ECG features into discrete, compact, and clinically meaningful local \texttt{rhythm codes}. These codes encapsulate basic morphological, frequency, and demographic information (\textit{e.g.}, sex), effectively mitigating signal noise. We further pre-train the {\model} to learn rhythmic pattern associations across ECG tokens, enabling the capture of cardiac event semantics.
By being jointly pre-trained on diverse ECG data sources, {\model} is capable of generalizing across a wide range of downstream tasks where ECG signals are recorded from various devices and scenarios. Experimental results in anomaly detection, arrhythmia detection, corrupted lead generation, and ultra-long ECG signal analysis demonstrate that {\model} learns common ECG knowledge from data and significantly outperforms cutting-edge methods in each respective task.

% such as anomaly detection, arrhythmia detection, missing channel generation, and lengthy ECG analysis. Extensive experiments show that {\model} consistently delivers outstanding performance in these tasks and demonstrates strong generalization across diverse ECG datasets.

% Experiments on abnormal detection, Arrhythmia classification, ECG lead generation, and identification of ultra-long ECG signals show that our \model outperforms all compared SOTA methods in their respective fields.

% For example, {\model} achieved over a 3\% improvement in accuracy compared to state-of-the-art methods in anomaly detection.




% ECGFM unifies heterogeneous data — accounting for variations in equipment, signal properties, lead configurations, sampling frequencies, and patient demographics — by transforming them into unified tokens.  Specifically, we segment ECG signals from different datasets into patches of uniform length to eliminate the effects of heterogeneity. Nonetheless, the challenge of noise within ECG patches persists due to the low SNR. To tackle this, we design a novel ECG tokenizer that converts noisy, continuous ECG patches into compact and meaningful tokens. The ECG tokenizer employs a discretization process that maps continuous signal segments into a finite set of code indices, guided by a proxy task that focuses on the intrinsic origins of ECG signals， effectively capturing essential signal patterns while suppressing noise. . 
% Subsequently, we pre-train ECGFM by predicting the code indices of masked tokens, allowing the model to learn the underlying meanings and relationships  while effectively disregarding noise. This approach enhances ECGFM's ability to generalize across diverse datasets. In downstream tasks such as arrhythmia classification and diagnosis, ECGFM consistently surpasses baseline models, demonstrating superior generalization and performance. Experimental results validate the model’s effectiveness in managing diverse ECG datasets. The code for ECGFM is available at XXX.

\end{abstract}

==> sec/3.related_work.tex <==
\section{Related Work}

\textbf{Heterogeneous ECG Signal Analysis and Classification}

% Recent advancements in deep learning have significantly improved the accuracy of ECG signal analysis and classification. Various architectures—particularly convolutional neural networks (CNNs), recurrent neural networks (RNNs), and transformer-based models—have been employed to automatically extract features from ECG signals and classify different types of arrhythmias without relying on hand-crafted features. One-dimensional CNNs (1D-CNNs) have been effective in detecting important patterns in ECG signals, enabling high-performance arrhythmia classification \cite{srivastava2023apneanet, jasvitha20241d, ribeiro2020automatic, gao2021end}. They have been successfully applied to datasets like PTB-XL for ECG signal classification \cite{prathipati2023combining, kucukseymen2022left} and have shown promising results in anomaly detection within physiological signals \cite{qin2023novel}.

% Meanwhile, RNNs, especially Long Short-Term Memory (LSTM) networks and Gated Recurrent Units (GRUs), excel at capturing temporal dependencies in ECG signals. These models are well-suited for detecting time-dependent irregularities such as atrial fibrillation and other heart rhythm abnormalities \cite{kumar2023investigation, din2024ecg}. LSTMs have been applied to tasks like R-peak detection \cite{karri2023real}, heart disease classification \cite{jafari2023automated}, arrhythmia identification \cite{goswami2023electrocardiogram}, atrial fibrillation detection \cite{phukan2023afibri}, congestive heart failure detection \cite{musa2023systematic}, and continuous heartbeat classification \cite{lim2024ecg}.

% Transformer architectures have gained attention in ECG analysis due to their ability to model long-range dependencies and handle sequential data effectively. Transformers leverage self-attention mechanisms to capture both local and global features, making them suitable for complex ECG signal analysis. Studies have shown that transformer-based models outperform traditional CNNs and RNNs in tasks such as arrhythmia detection and ECG signal classification \cite{shah2024ecg, ji2024msgformer}. They have also been applied in detecting myocardial infarction and other cardiac abnormalities with promising results \cite{vaid2023foundational, li2024clinical}.

% However, most existing models are trained on homogeneous datasets with consistent lead configurations, signal lengths, and sampling frequencies. This homogeneity poses challenges when applying these models to heterogeneous data, where variations in signal quality, noise levels, and lead setups are common. Therefore, there is a pressing need for models capable of handling heterogeneous data effectively, especially in environments with limited labels or high noise levels.

The application of deep learning techniques has significantly advanced the analysis and classification of ECG signals. However, a fundamental issue persists: many ECG datasets are small and heterogeneous, varying in lead configurations, signal lengths, and sampling frequencies. This diversity has hindered the development of a unified model, as models trained on one dataset often do not generalize well to others. Consequently, researchers have focused on designing specialized models tailored to specific datasets, employing architectures like convolutional neural networks (CNNs), recurrent neural networks (RNNs), and transformer-based models. While these efforts have led to incremental performance improvements \cite{srivastava2023apneanet, jasvitha20241d, ribeiro2020automatic, gao2021end}, the gains are often not statistically significant due to the limited size and scope of the datasets used. For instance, 1D-CNNs have shown effectiveness in detecting patterns within specific datasets like PTB-XL \cite{prathipati2023combining, kucukseymen2022left}, but their applicability remains constrained to the conditions under which they were trained. RNNs, particularly Long Short-Term Memory (LSTM) networks and Gated Recurrent Units (GRUs), have been utilized to capture temporal dependencies in ECG signals \cite{kumar2023investigation, din2024ecg}. However, their performance gains are modest and often dataset-specific. Transformer-based models have recently gained attention for their ability to model long-range dependencies \cite{shah2024ecg, ji2024msgformer}, yet they too face difficulties in generalizing across datasets with different characteristics. The absence of a unified model that can handle the heterogeneity of ECG data underscores the need for approaches that can deliver more significant and broadly applicable performance improvements.


\textbf{Self-supervised ECG Representation Learning}
% In recent years, self-supervised learning has emerged as a powerful paradigm for learning representations from unlabeled ECG data, enabling models to leverage vast amounts of ECG signals without the need for costly manual annotations. Typically, these methods involve pretraining a model on large datasets using tasks such as signal reconstruction, contrastive learning, or masked signal modeling. Once pretrained, the model can be fine-tuned on smaller, labeled datasets to achieve high accuracy in specific tasks like arrhythmia classification or anomaly detection \cite{yun2024automatic, wu2024improving}.

% Several self-supervised learning approaches have been developed specifically for 12-lead ECG data. For instance, Kiyasseh and Zhu \cite{kiyasseh2021clocs} proposed Contrastive Multi-Segment Coding (CMSC), a contrastive method that divides an ECG signal into segments, encouraging similar representations for compatible segments while pushing apart incompatible ones. Contrastive Predictive Coding (CPC) \cite{mehari2022self} has also been applied to ECG data, where the model predicts future representations of the signal. However, CPC faces scalability issues with large datasets due to the computational overhead of LSTM modules, making training extremely slow.

% Masked signal modeling has also shown promise in ECG representation learning. Zhang et al. \cite{zhang2022maefe} introduced masked autoencoders for ECG data, incorporating temporal and channel-based masking techniques known as the Masked Time Autoencoder (MTAE) and Masked Lead Autoencoder (MLAE). Similarly, Na et al. \cite{na2024guiding} developed ST-MEM, a masked autoencoder that applies random time interval masking across different leads. A potential limitation of methods like MLAE and ST-MEM is that predicting certain patches can be relatively straightforward due to the high correlation among the 12-lead signals.

% Despite these advancements, several challenges remain. Current self-supervised methods often lack strong generalization capabilities across different ECG datasets, especially when confronted with varying lead configurations and noise levels.  The low signal-to-noise ratio (SNR) inherent in ECG data can lead models to capture excessive noise instead of critical physiological information, impairing their ability to focus on relevant features.  Consequently, these models struggle to extract meaningful representations that transfer well to unseen data or datasets with different characteristics, resulting in poor generalization performance.


Self-supervised learning has emerged as a promising approach for learning representations from unlabeled ECG signals, enabling the utilization of large amounts of data without the need for manual annotations. Methods such as signal reconstruction, contrastive learning, and masked signal modeling have been explored \cite{yun2024automatic, wu2024improving,li2024learning}. While these approaches leverage large amounts of data for pretraining, they have not sufficiently addressed key limitations.

Existing methods often do not generalize well across heterogeneous ECG datasets, particularly when faced with varying lead configurations and noise levels. For example, contrastive methods\cite{kiyasseh2021clocs,wang2023adversarial} encourage similar representations for compatible signal segments but do not adequately account for the variability introduced by different lead setups.  Moreover, the low SNR inherent in ECG data can cause models to focus on reconstructing noisy or redundant signal components due to high correlations among leads, rather than capturing critical physiological information. Models like CPC \cite{mehari2022self} and masked autoencoders \cite{zhang2022maefe, na2024guiding} may inadvertently emphasize less relevant features, which diminishes their effectiveness in capturing essential signal characteristics. This focus on less informative aspects of the data can limit the models' ability to extract meaningful representations that transfer effectively to unseen data or datasets with different characteristics.

As a result of these unaddressed limitations—including the difficulty in generalizing across diverse datasets and the challenge posed by low SNR leading to less transferable representations—the performance gains achieved by existing self-supervised methods remain modest. There is a pressing need for models that can effectively handle the heterogeneity of ECG data, focus on capturing essential physiological information despite noise, and extract representations that generalize well across diverse datasets.


% \section{Notations}
% \label{sec:appx_notation}

% \xunote{Update all notations here:}

% \begin{table*}[h]
%     \centering
%     \renewcommand{\arraystretch}{1.2}
%     \adjustbox{max width=\textwidth}{ 
%     \begin{tabular}{p{3cm} p{10cm}}
%     \hline
%     \multicolumn{2}{l}{\textbf{Special Tokens}} \\
%     \hline
%     $[CLS]$ & Start of sequence token \\
%     $[VS], [VE]$ & Start of visit and end of visit tokens \\
%     $[REG]$ & Register token \\
%     $[W_0]$ to $[W_3]$ & Week tokens (indicating different weeks) \\
%     $[M_0]$ to $[M_{12}]$ & Month tokens (indicating different months) \\
%     $[LT]$ & Long-term time interval token \\
%     $[PAD]$ & Padding token \\
%     $[UNK]$ & Unknown token \\
%     $[MASK]$ & Mask token \\
%     \hline
%     \multicolumn{2}{l}{\textbf{Event Tokens and Attributes}} \\
%     \hline
%     $e_{v,j}$ & Event token at visit $v$, index $j$ \\
%     $\tau_{v,j}$ & Timestamp of the event $e_{v,j}$ \\
%     $T$ & Type of event (procedure (P), medication (M), or lab result (L)) \\
%     $A$ & Age of the patient at the time of the event \\
%     $S$ & Visit segment, indicating the separation between adjacent visits \\
%     $V$ & Visit order, visit number incrementing for each subsequent visit \\
%     $\mathcal{P}$ & Absolute position of the event within the sequence \\
%     \hline
%     \multicolumn{2}{l}{\textbf{Functions and Mappings}} \\
%     \hline
%     $f(e_{v,j})$ & Function mapping the event space $\mathcal{E}$ to a set of attributes $\Gamma$ \\
%     $\mathcal{C}(v,j)$ & Context of the token $e_{v,j}$ \\
%     $\mathcal{M}$ & Set of masked indices for Masked Language Modeling (MLM) \\
%     $\mathcal{I}$ & Indices for Next Token Prediction (NTP) task \\
%     \hline
%     \multicolumn{2}{l}{\textbf{Model Parameters and Objectives}} \\
%     \hline
%     $\theta, \mathcal{D}$ & Model parameters and Dataset \\
%     $y, \hat{y}(x; \theta)$ & Actual and Predicted clinical outcomes \\
%     $\mathcal{L}_i$ & Binary cross-entropy loss for task $c_i$ \\
%     \hline
%     \multicolumn{2}{l}{\textbf{Embedding Layer}} \\
%     \hline
%     $E_{v,j}$ & Embedding of event token $e_{v,j}$ \\
%     $E_{\text{concept}}(e_{v,j})$ & Concept embedding of event token $e_{v,j}$ \\
%     $E_{\text{type}}(T_{v,j})$ & Token type embedding of event token $T_{v,j}$ \\
%     $E_{\text{age}}(A_{v,j})$ & Age embedding of event token $A_{v,j}$ \\
%     $E_{\text{time}}(\tau_{v,j})$ & Time embedding of event token $\tau_{v,j}$ \\
%     $E_{\text{segment}}(S_{v,j})$ & Segment embedding of event token $S_{v,j}$ \\
%     $E_{\text{visit order}}(V_{v,j})$ & Visit order embedding of event token $V_{v,j}$ \\
%     $E_{\text{position}}(\mathcal{P}_{v,j})$ & Positional embedding of event token $\mathcal{P}_{v,j}$ \\
%     \hline
%     \end{tabular}
%     }
% \end{table*}
% \vspace{0pt}







==> sec/4.methodology.tex <==
\section{Methodology}
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{fig/structure5.pdf}
    \caption{\textbf{Overall architecture and pre-training pipeline of ECGFM.} 
    % The architecture comprises two main components: Patient Attribute Tokenizer Training and the ECGFM Model Structure. 
    % ECGFM is pre-trained in two steps. The Patient Attribute Tokenizer is pre-trained through proxy tasks to embed morphology, frequency, and patient attributes into tokens \textbf{(Up)}. The entire ECGFM, along with the Patient Attribute Tokenizer, is further pre-trained using code index supervision for ... Additionally, a complementary masking approach is employed to...
    % A complementary masking approach is . (\textbf{down})
    % During pre-training, complementary masking ECG signals are processed using the pretrained tokenizer to perform code prediction, thereby preparing the model for downstream tasks.
    % The structure is divided into two main components: Patient Attribute Tokenizer Training and ECGFM Pre-training. In Patient Attribute Tokenizer Training, ECG signals are encoded temporally and spatially into feature vectors, which are then quantized for reconstruction and attribute prediction. In ECGFM Pre-training, masked ECG signals are used for pre-training, where token prediction and classification tasks are performed for downstream tasks.
    ECGFM is pre-trained in two steps. The Patient Attribute Tokenizer is pre-trained through proxy tasks to embed morphology, frequency, and demography into tokens \textbf{(Up)}. Then, the entire ECGFM, along with the Patient Attribute Tokenizer, is further pre-trained by predicting the code indices of the masked tokens to learn the semantic relationships between tokens \textbf{(Down)}. 
    % Additionally, a complementary masking approach was proposed to provide more masking perspectives focusing on both heavily masked and minimally masked regions of the ECG signals.
    }
    \label{fig:main}
\end{figure*}


The overarching goal in ECG signal representation learning is to design new tokenizers that can be adapted to the self-supervised learning pipeline as well as multiple downstream tasks. Thus, we proposed ECGFM. As illustrated in Figure~\ref{fig:main}, The structure of ECGFM is divided into three main components: the \tokenizer, Temporal Encoder, and Fourier Spectrum Prediction. We will explain how the signals flow between these components: ECG signals are first tokenized into patches, then encoded temporally, and finally fed into a prediction module for downstream tasks. Subsequent steps will detail each process in more depth.

% In this section, we provide a detailed explanation of the entire framework of ECGFM. We first represent the multi-channel ECG signals as \( X \in \mathbb{R}^{C \times T} \), where \( C \) is the number of ECG leads (channels), and \( T \) represents the total number of time steps.


 % The set of electrodes for \( X \) is denoted as \( C_X = \{c_{i1}, c_{i2}, ..., c_{iC}\} \), where \( C_X \subseteq C = \{c_1, c_2, ..., c_{|C|}\} \), and \( C \) represents the general set of channels used in ECG signal collection, corresponding to a standard 12-lead ECG setup. We explain how the signals from these channels are processed and utilized in our model.

% \subsection{ECGFM Architecture}

% We propose ECGFM, a generalized architecture for representing ECG signals. It is designed to handle any input ECG signal, regardless of the number of channels or the length of the time series, as illustrated in Figure 1. 


\subsection{Patient Attribute-Aligned Tokenization}

The multi-channel ECG signals can be represented as \( X \in \mathbb{R}^{C \times T} \), where \( C \) is the number of ECG leads (channels), and \( T \) is the total number of time steps. To efficiently preprocess the ECG signals $X$, we segment the signals into patches of equal length along the time axis. Each patch has a length of \( w \) time steps, resulting in \( P = \left\lceil  \frac{T}{w} \right\rceil  \) patches per lead. Each patch is denoted as \( x_{j,k} \in \mathbb{R}^{w} \), where \( j = 1, 2, ..., C \) represents the lead index and \( k = 1, 2, ..., P \) represents the patch index along the time axis. Therefore, the set of all patches is \( \{ x_{j,k} \in \mathbb{R}^{w} \mid j = 1, 2, ..., C; \, k = 1, 2, ..., P \} \), and the total number of patches is \( C \times P = C \left\lceil \frac{T}{w} \right\rceil \).




% \subsubsection{Temporal Encoder}

% To address the temporal nature of ECG signals, we employ a temporal encoder that captures time dependencies and sequences. The temporal encoder processes the segmented patches to capture the dynamic patterns over time. By aggregating information from these patches, we create a representation that emphasizes both short-term and long-term dependencies in the ECG signal. This step is crucial for detecting irregularities such as arrhythmias.

\subsubsection{Temporal-Spatial Embedding}

% In this step, we embed both the temporal and spatial dimensions of the ECG data into a unified representation. The temporal embedding encodes the position of each patch in time, while the spatial embedding captures the relationships between different ECG channels. These embeddings allow the model to learn both the rhythm and spatial dependencies between channels, improving the ability to generalize across varying channel configurations and signal lengths.


To effectively capture both temporal and spatial characteristics of ECG signals, we employ a temporal-spatial embedding approach. This method enables the model to process complex ECG data by integrating dynamic temporal patterns and spatial relationships between different leads.

Since ECG signals are highly time-sensitive, it is crucial to first extract temporal dependencies. We achieve this by using a temporal encoder that processes each ECG patch $x_{j,k}$ through a series of convolutional layers. These layers consist of 1D convolutions, group normalization, and GELU activation functions, transforming the raw signal into temporal embeddings. The output of the temporal encoder for each patch can be described as:

\begin{equation}
\begin{aligned}
e = \{ e_{j,k} \in \mathbb{R}^d \mid j = 1, 2, \dots, C; \, k = 1, 2, \dots, P \}
\end{aligned}
\end{equation}

% where \( e_{c_{ij}, k} \) represents the embedding for each ECG patch, \( d \) is the dimension of the embeddings, \( C \) is the number of ECG leads, and \( w \) is the window length. To enhance the model's understanding of the temporal sequence, learnable temporal embeddings are added to encode the positional information for each time step.

where \( e_{j,k} \) represents the embedding for each ECG patch \( x_{j,k} \), \( d \) is the dimension of the embeddings, \( C \) is the number of ECG leads, and \( P = \left\lceil \frac{T}{w} \right\rceil \) is the number of patches per lead. To enhance the model's understanding of the temporal sequence, learnable temporal embeddings \( te_k \in \mathbb{R}^d \) are added to encode the positional information for each time step \( k \).


In addition to the temporal dimension, the spatial relationships between different ECG leads are critical for a comprehensive understanding of the signals. Each ECG lead \( j \) is associated with a spatial embedding \( se_j \in \mathbb{R}^d \), allowing the model to capture the interactions between leads. The combination of temporal and spatial embeddings is applied as:

\begin{equation}
\begin{aligned}
\hat{e}_{j,k} = e_{j,k} + te_k + se_j
\end{aligned}
\end{equation}

where \( te_k \) and \( se_j \) are the temporal and spatial embeddings, respectively. This combination allows the model to capture both time-dependent features and the spatial dependencies across different leads.


% In addition, in order to pay more attention to the relationship between each patch in the same lead and the relationship between patches in different leads at the same time. We introduce **Cross-Pattern Attention (CroPA)**, a masked self-attention mechanism designed specifically for multi-lead ECG data. CroPA allows each patch to attend only to patches within the same lead and temporal space, ensuring the model focuses on relevant temporal and spatial patterns, while disregarding unrelated patches from different leads and times. This is an improvement over standard attention mechanisms, where patches attend to all other patches indiscriminately. The CroPA mechanism is computed as:
% \[
% \text{CroPA}(Q, K, V) = \text{softmax}\left(\frac{\text{LN}(Q) \cdot \text{LN}(K)^T + M}{\sqrt{d_{\text{head}}}}\right) V
% \]
% where \( Q \), \( K \), and \( V \) are the query, key, and value matrices, and \( d_{\text{head}} \) is the dimensionality of each attention head. By restricting attention within relevant patches, CroPA enhances the model’s ability to capture consistent patterns across ECG leads, making it more effective in identifying cardiac abnormalities.

% After processing the embeddings through multiple layers of CroPA, the final output is aggregated and used for downstream tasks. This temporal-spatial embedding strategy, combined with CroPA, enables the model to capture both short-term temporal dynamics and long-range spatial relationships between ECG leads, leading to more accurate ECG analysis.

Given that biological signals, particularly ECG data, often require simultaneous observation across multiple leads, interpreting a single patch must consider other patches within the same channel and across different channels. In a 12-lead ECG, for instance, abnormalities must be consistent across multiple leads to diagnose specific cardiac pathologies. To address this, we introduce \textbf{Cross-Patch Attention (CPA)}, a masked self-attention mechanism designed specifically for multi-lead ECG data.

CPA allows each patch to attend only to patches within relevant spatial and temporal contexts, ensuring the model focuses on pertinent temporal and spatial patterns while disregarding unrelated patches from different leads and times. This is an improvement over standard attention mechanisms, where patches attend to all other patches indiscriminately.

Formally, let \( \hat{E} \in \mathbb{R}^{N \times d} \) be the matrix of embeddings, where \( N = C \times P \) is the total number of patches, \( d \) is the embedding dimension, and \( \hat{E} \) is constructed by stacking the embeddings \( \hat{e}_{j,k} \) for all leads \( j = 1, 2, ..., C \) and patch indices \( k = 1, 2, ..., P \). The embeddings are flattened in a consistent order, such as by iterating over all patches in each lead sequentially.
We compute the query, key, and value matrices as:
\[
Q = \text{LayerNorm}(\hat{E}) W_Q, \quad K = \text{LayerNorm}(\hat{E}) W_K, \quad V = \hat{E} W_V
\]
where, \( W_Q, W_K, W_V \in \mathbb{R}^{d \times d_{\text{model}}} \) are learnable projection matrices,
\( \text{LayerNorm}(\cdot) \) denotes Layer Normalization applied to each embedding,
\( d_{\text{model}} \) is the model dimension. The CPA mechanism is then computed as:


\begin{equation}
\begin{aligned}
\text{CPA}(Q, K, V) = \text{softmax}\left( \frac{Q K^\top + M}{\sqrt{d_{\text{head}}}} \right) V
\end{aligned}
\end{equation}

where, \( M \in \mathbb{R}^{N \times N} \) is the attention mask matrix defined by:

\begin{equation}
\begin{aligned}
M_{i,j} = \begin{cases}
0, & \text{if } j \in \mathcal{A}(i) \\
-\infty, & \text{otherwise}
\end{cases}
\end{aligned}
\end{equation}

 \( \mathcal{A}(i) \) includes patches within the same lead \( j \) and neighboring leads, and within a specified temporal window around the patch \( k \).
By constructing \( M \) in this way, we ensure that each patch attends only to relevant patches, enhancing the model's ability to capture consistent patterns across ECG leads.

\subsubsection{\tokenizer}

ECG signals are inherently high-dimensional and time-series data, but they are often characterized by a low signal-to-noise ratio (SNR) due to the fact that useful information is often sparse in the data. Moreover, ECG data is plagued by various types of noise, which can originate from different equipment, patient demographics, data collection methods, and even variations across datasets. These issues lead to significant attribute distribution discrepancies between different ECG datasets, making it difficult to effectively train generalizable models. To address the challenge of the lack of an effective ECG representation learning paradigm, we propose a neural tokenizer to transform raw ECG signals into discrete tokens, facilitating robust and noise-resistant representation learning. Our approach involves the use of a vector-quantized neural tokenizer, designed to transform the continuous, noisy ECG signals into compact, discrete tokens that represent the underlying physiological patterns. By doing so, we convert low-SNR signals into a high-SNR representation that accurately reflects the real cardiac activity while mitigating the impact of noise.

First, each patch \( x_{j,k} \in \mathbb{R}^w \) represents a portion of the signal over \( w \) time steps in lead \( j \). The tokenizer processes these patches into feature representations, yielding embeddings \( e_{j,k} \in \mathbb{R}^d \), where \( d \) is the dimension of each embedding. These embeddings are then mapped to discrete tokens using a quantizer. Specifically, the quantizer selects the closest token from a predefined codebook \( V = \{ v_i \in \mathbb{R}^D \mid i = 1, 2, \dots, K \} \), \( K \) is the number of discrete codebook vectors,
 \( D \) is the dimension of each codebook vector.

The tokenization process is described mathematically as follows: For each embedding \( e_{j,k} \), the quantizer selects the nearest codebook vector \( v_{i^\ast} \) by minimizing the distance between the normalized embedding and the normalized codebook vectors:

\[
i^\ast = \arg \min_{i} \left\| \frac{e_{j,k}}{\| e_{j,k} \|_2} - \frac{v_i}{\| v_i \|_2} \right\|^2
\]

where \( \| \cdot \|_2 \) denotes the \( \ell_2 \)-norm, and normalization ensures that the distance measure is equivalent to maximizing the cosine similarity.

The assigned discrete token for the patch \( x_{j,k} \) is then the index \( i^\ast \):
\[
z_{j,k} = i^\ast
\]


This process effectively quantizes the ECG signal into a sequence of discrete tokens \( \{ z_{j,k} \} \), reducing the influence of noise and enhancing the signal quality.

By transforming the ECG data into high-SNR tokenized representations \( z_{j,k} \), the neural tokenizer enables the model to focus on the meaningful aspects of the cardiac signal, such as heartbeat patterns and rhythms. These discrete tokens correspond to the real-time electrical activity of the heart, allowing for more accurate analysis and interpretation of the data. This approach improves the model’s ability to generalize across different datasets, even when there are variations in data collection methods, patient demographics, and equipment.


In summary, our neural tokenizer addresses the challenges posed by the inherent low-SNR and high-dimensional nature of ECG data, as well as the variations between datasets. By converting the raw signals into discrete, high-SNR tokens that reflect real cardiac events, we create a more robust and generalizable representation for downstream tasks such as anomaly detection and rhythm classification.

% \subsubsection{Codebook}

% The Codebook component is responsible for creating a dictionary of common signal patterns found in ECG data. This dictionary allows for efficient compression and representation of ECG signals, reducing redundancy while preserving critical information necessary for accurate diagnosis.

\subsubsection{Fourier Spectrum Prediction}

% To enhance the model’s ability to capture frequency-domain characteristics of ECG signals, we introduce a Fourier Spectrum Prediction module. This component predicts the frequency spectrum of the ECG signals, which is particularly useful in identifying rhythm disorders such as atrial fibrillation that manifest in both time and frequency domains.

To address the challenges of low signal-to-noise ratio (SNR) and various types of noise in ECG signals, we propose a Fourier spectrum-based prediction approach. This method aims to capture both the original temporal signals and their corresponding frequency characteristics, transforming raw ECG data into a more robust representation that emphasizes meaningful cardiac activity.

Unlike traditional methods that focus solely on time-domain features, our approach leverages the Discrete Fourier Transform (DFT) to incorporate both temporal and frequency domains of the ECG signals. This allows us to better account for periodic patterns that are crucial in analyzing heartbeats and diagnosing cardiac conditions.

For each ECG patch \( x_{j,k} \in \mathbb{R}^w \) from lead \( j \) at patch index \( k \), we apply the DFT to convert the time-domain signal into its frequency components. The transformation is defined as follows:

\[
\tilde{x}_{j,k}[m] = \sum_{n=0}^{w-1} x_{j,k}[n] \cdot e^{-i 2\pi m n / w}, \quad m = 0, 1, \dots, w-1
\]
where  \( i \) is the imaginary unit, \( \tilde{x}_{j,k}[m] \) represents the complex frequency component at frequency index \( m \), \( n \) is the time index within the patch.

We calculate the frequency magnitude \( f_{j,k}[m] \) for each frequency component \( m \) as:
\[
f_{j,k}[m] = \left| \tilde{x}_{j,k}[m] \right| = \sqrt{ \left( \text{Re}(\tilde{x}_{j,k}[m]) \right)^2 + \left( \text{Im}(\tilde{x}_{j,k}[m]) \right)^2 }
\]
where \( \text{Re}(\cdot) \) and \( \text{Im}(\cdot) \) denote the real and imaginary parts, respectively. For stable convergence during training, we apply z-score normalization to the frequency magnitudes within each patch.

% Once the ECG patches are transformed into the frequency domain, we quantize them using a codebook \( V \) to produce a compact and high-SNR representation of the cardiac signal. Each normalized patch representation \( \ell_2(z_i) \) is matched to the nearest codebook embedding \( v_j \), forming a set of tokens that represent the cardiac activity. 

In addition to transforming the ECG signals into robust temporal-frequency tokens, we also incorporate the prediction of patient-specific attributes (e.g., age, weight, or other demographic factors). These attributes, represented as a vector \( a \in \mathbb{R}^{d_a} \), are jointly predicted alongside the temporal and frequency information to enhance the model's understanding of the patient's specific condition. This personalized aspect allows the model to better account for inter-patient variability, which is critical in making accurate clinical predictions.

The learning objective for this task involves minimizing a combination of reconstruction loss, codebook loss, and commitment loss. The overall loss function is formulated as:
\[
\begin{aligned}
\mathcal{L}_1 = &\sum_{j=1}^{C} \sum_{k=1}^{P} \left( \left\| o_{j,k}^t - x_{j,k} \right\|_2^2 + \left\| o_{j,k}^f - f_{j,k} \right\|_2^2 \right) \\
&+ \sum_{j=1}^{C} \sum_{k=1}^{P} \left( \left\| \text{sg}\left( e_{j,k} \right) - v_{z_{j,k}} \right\|_2^2 + \beta \left\| e_{j,k} - \text{sg}\left( v_{z_{j,k}} \right) \right\|_2^2 \right) \\
&+ \left\| o^a - a \right\|_2^2
\end{aligned}
\]

% where \( o_i^t \) and \( o_i^f \) are the outputs of the temporal and frequency decoders, respectively, and \( o_i^a \) represents the predicted patient-specific attributes. The loss function balances the reconstruction of both the temporal and frequency components of the ECG signal while ensuring that the quantized tokens remain faithful to the original signal and incorporate patient-specific factors.

where \( o_{j,k}^t \) and \( o_{j,k}^f \) are the outputs of the temporal and frequency decoders for patch \( x_{j,k} \). respectively, \( e_{j,k} \) is the embedding of the patch \( x_{j,k} \),  \( v_{z_{j,k}} \) is the codebook vector corresponding to the token \( z_{j,k} \). \( \text{sg}(\cdot) \) denotes the stop-gradient operator. \( \beta \) is a weighting coefficient for the commitment loss and   \( o^a \) represents the predicted patient-specific attributes,  \( a \) is the ground truth patient attribute vector. The loss function balances the reconstruction of both the temporal and frequency components of the ECG signal while ensuring that the quantized tokens remain faithful to the original signal and incorporate patient-specific factors.




\subsection{ECGFM Pre-training}

\subsubsection{Masked ECG Modeling}

Inspired by masked language models, we adopt a Masked ECG Modeling approach, where random segments of ECG signals are masked and the model is tasked with reconstructing the missing parts. This self-supervised learning technique helps the model learn robust representations of ECG signals by capturing complex temporal dependencies and patterns.

\subsubsection{Mirror Masking}

% We apply symmetric masking across multiple ECG channels, ensuring that the model learns to infer the missing parts in a way that preserves the inter-channel relationships, which are crucial for diagnosing multi-lead ECG data.
% ### Symmetric Regression Masking

To address the challenge of learning robust ECG representations, we introduce a Symmetric Regression Masking approach. This method builds upon masked ECG modeling and multi-channel autoregressive strategies, combining the strengths of both techniques to better capture temporal and spatial dependencies across ECG leads.

In our approach, the temporal encoder processes each patch \( x_{j,k} \) to obtain embeddings \( e_{j,k} \in \mathbb{R}^d \). A mask \( \mathcal{M} = \{ m_{j,k} \mid j = 1, \dots, C; \, k = 1, \dots, P \} \) is then generated, where \( m_{j,k} \in \{0, 1\} \), and a proportion \( r \) of the patches are masked (\( m_{j,k} = 1 \)). The masked patches are replaced with a learnable mask token \( e_M \in \mathbb{R}^d \). The masked embeddings \( \hat{e}_{j,k} \) are defined as:
\[
\hat{e}_{j,k} = \begin{cases}
e_{j,k}, & \text{if } m_{j,k} = 0 \\
e_M, & \text{if } m_{j,k} = 1
\end{cases}
\]
These embeddings are then augmented with temporal and spatial positional embeddings:
\[
\tilde{e}_{j,k} = \hat{e}_{j,k} + te_k + se_j
\]

where \( te_k \in \mathbb{R}^d \) is the temporal positional embedding for patch \( k \), \( se_j \in \mathbb{R}^d \) is the spatial positional embedding for lead \( j \).

The combined embeddings \( \tilde{e}_{j,k} \) are then flattened into a sequence and fed into a transformer encoder to generate hidden representations \( h_{j,k} \in \mathbb{R}^d \).


For prediction, each hidden vector \( h_{j,k} \) is passed through a linear classifier to produce the probability distribution over the codebook tokens \( V = \{ v_i \in \mathbb{R}^D \mid i = 1, 2, \dots, K \} \):
\[
p(v_i \mid \tilde{E}) = \text{softmax}\left( \text{Linear}(h_{j,k}) \right)
\]
where \( \tilde{E} \) is the set of all \( \tilde{e}_{j,k} \).

The training objective for the masked modeling process is to minimize the negative log-likelihood of predicting the correct tokens \( v_{z_{j,k}} \) at the masked positions:
\[
\mathcal{L}_\text{mask} = - \sum_{j=1}^{C} \sum_{k=1}^{P} m_{j,k} \cdot \log p\left( v_{z_{j,k}} \mid \tilde{E} \right)
\]


In addition to the masked modeling, we integrate an autoregressive component to enhance the temporal dependencies between ECG patches. ECG signals vary across leads and are inherently multi-dimensional. Therefore, we adopt a multi-lead autoregressive strategy, where each token in a specific lead predicts the next token within the same lead, while also considering tokens from other leads at previous and current time steps.

The probability of predicting the sequence of tokens \( \{ z_{j,k} \} \) for all leads \( j = 1, \dots, C \) and patches \( k = 1, \dots, P \) is formulated as:

\[
p\left( \{ z_{j,k} \} \right) = \prod_{k=1}^{P} \prod_{j=1}^{C} p\left( z_{j,k} \mid \text{context}_{j,k} \right)
\]

where \( \text{context}_{j,k} \) includes:
All tokens \( \{ z_{j',k'} \} \) such that \( k' < k \) for all leads \( j' = 1, \dots, C \),
Tokens \( \{ z_{j',k} \} \) for leads \( j' < j \) at the current time step \( k \).

To implement this, we define a staircase mask \( M \in \mathbb{R}^{N \times N} \) (with \( N = C \times P \)) that allows each token \( z_{j,k} \) to attend to the specified context. The mask \( M \) is constructed such that:
\[
M_{(j,k),(j',k')} = \begin{cases}
0, & \text{if } (k' < k) \text{ or } (k' = k \text{ and } j' < j) \\
-\infty, & \text{otherwise}
\end{cases}
\]

This mask ensures that when predicting token \( z_{j,k} \), the model attends to: all tokens from all leads at previous time steps and tokens from earlier leads at the current time step.

The training objective for the autoregressive component is to minimize the negative log-likelihood:
\[
\mathcal{L}_\text{ar} = - \sum_{j=1}^{C} \sum_{k=1}^{P} \log p\left( v_{z_{j,k}} \mid \text{context}_{j,k} \right)
\]

The overall loss function combines both the masked modeling loss and the autoregressive loss:
\[
\mathcal{L} = \mathcal{L}_\text{mask} + \mathcal{L}_\text{ar}
\]

By combining the masked prediction and autoregressive strategies, the Symmetric Regression Masking approach effectively enhances the model's ability to learn robust ECG representations. This approach ensures that temporal dependencies are maintained while also capturing the spatial interactions between ECG leads, resulting in improved generalization and performance across various ECG analysis tasks.

\subsubsection{Linear Attention Encoder}

Finally, we use a linear attention encoder to reduce the computational complexity of the model. This encoder is designed to handle long sequences efficiently, making it suitable for real-time ECG analysis in clinical settings. The linear attention mechanism helps the model focus on critical signal patterns while discarding irrelevant noise.

==> sec/content.tex <==

% \tableofcontents
